MedGNN: Towards Multi-resolution Spatiotemporal Graph Learning for Medical Time Series Classification

Medical time series has been playing a vital role in real-world healthcare systems as valuable information in monitoring health conditions of patients. Accurate classification for medical time series, e.g., Electrocardiography (ECG) signals, can help for early detection and diagnosis. Traditional methods towards medical time series classification rely on handcrafted feature extraction and statistical methods; with the recent advancement of artificial intelligence, the machine learning and deep learning methods have become more popular. However, existing methods often fail to fully model the complex spatial dynamics under different scales, which ignore the dynamic multi-resolution spatial and temporal joint inter-dependencies. Moreover, they are less likely to consider the special baseline wander problem as well as the multi-view characteristics of medical time series, which largely hinders their prediction performance. To address these limitations, we propose a Multi-resolution Spatiotemporal Graph Learning framework, MedGNN, for medical time series classification. Specifically, we first propose to construct multi-resolution adaptive graph structures to learn dynamic multi-scale embeddings. Then, to address the baseline wander problem, we propose Difference Attention Networks to operate self-attention mechanisms on the finite difference for temporal modeling. Moreover, to learn the multi-view characteristics, we utilize the Frequency Convolution Networks to capture complementary information of medical time series from the frequency domain. In addition, we introduce the Multi-resolution Graph Transformer architecture to model the dynamic dependencies and fuse the information from different resolutions. Finally, we have conducted extensive experiments on multiple medical real-world datasets that demonstrate the superior performance of our method. Our Code is available.

==> tables/five_metrics.tex <==
\begin{table}[h]
\vspace{-3mm}
    \centering
    \caption{Summary of metrics.}
    \vspace{-3mm}
    \scalebox{0.9}{
    \begin{tabular}{c c c}
    \toprule[2pt]
       {Metrics}  &Formulas  &Explanations  \\
       \midrule
       {Accuracy} &\makecell[c]{$\frac{\text { TP }+ \text { TN }}{\text { All }}$} &\makecell[c]{Overall correctness \\of classifications.} \\
       {Precision} &\makecell[c]{$\frac{\text { TP }}{\text { TP }+ \text { FP }}$} &\makecell[c]{Correct positive classifications \\ out of all positive classifications.} \\
       {Recall} &\makecell[c]{$\frac{\text { TP }}{\text { TP }+ \text { FN}}$} &\makecell[c]{Correctly identified positives \\ from actual positives. }\\
       {F1 Score} &\makecell[c]{$2 \times \frac{\text { Precision } \times \text { Recall }}{\text { Precision }+ \text { Recall }}$} &\makecell[c]{Balance between \\ precision and recall.} \\
       AUROC &\makecell[c]{The area under \\ the ROC curve.} &\makecell[c]{Ability to distinguish \\ between classes.} \\
    \bottomrule[2pt]
    \end{tabular}
    }
    \label{tab:metrics}
    \vspace{-4mm}
\end{table}
